TauREx3 PhaseCurve: A 1.5D model for phase curve description

In the recent years, retrieval analysis of exoplanet atmospheres have been very successful, providing deep insights on the composition and the temperature structure of these worlds via the transit and eclipse methods. Analysis of spectral phase curve observations, which in theory provides even more information, are still limited to a few planets. In the next decade, new facilities such as NASA-JWST and ESA-Ariel will revolutionise the field of exoplanet atmospheres and we expect that a significant time will be spent on spectral phase curve observations. Most current models are still limited in their analysis of phase curve data as they do not consider the planet atmosphere as a whole or they require large computational resources. In this paper we present a semi-analytical model that will allow to compute exoplanet emission spectra at different phase angles. Our model provides a way to simulate a large number of observations while being only about 4 times slower than the traditional forward model for plane parallel primary eclipse. This model, which is based on the newly developed TauREx3 framework (Al-Refaie 2020), will be further developed to allow for phase curve atmospheric retrievals.

==> note.tex <==

TiO VO abundance given for W121b:
https://arxiv.org/pdf/0809.1865.pdf 





Choice of the Pressure point: \\

https://www.aanda.org/articles/aa/pdf/2014/04/aa22895-13.pdf has a pressure profile for HD209 and HD189 with a shift point of: \\
- NH3: 1e-2 Bar eg 1e3 Pa \\
- CH4 - CO: around 1 Bar eg 1e5 Pa \\ 
- HCN: 1e-2 Bar eg 1e3 Pa (but 3layer?) \\ \\

http://iopscience.iop.org/article/10.1088/0004-637X/737/1/15/pdf also shows that a lot of species shift around 1e-3 Bar eg 1e3 Pa \\ \\ 

http://iopscience.iop.org/article/10.3847/0004-637X/829/2/66/pdf this also shows that a lot of things happen around 1e3 Pa \\

https://www.aanda.org/articles/aa/pdf/2012/10/aa19310-12.pdf  \\
https://arxiv.org/pdf/1412.0930.pdf \\
http://iopscience.iop.org/article/10.1088/0004-637X/763/1/25/pdf \\ 
https://link.springer.com/content/pdf/10.1007%2Fs10686-014-9406-1.pdf \\

http://rsta.royalsocietypublishing.org/content/roypta/372/2014/20130073.full.pdf
